Revisiting the $DD^\ast$ chiral interactions with the local momentum-space regularization up to the third order and the nature of $T_{cc}^+$

We revisit the $DD^\ast$ interactions in chiral effective field theory up to the third order for the first time. We deal with the pion-exchanged interactions via local momentum-space regularization, in which we focus on their long-range behaviors through demanding their contributions vanish at the origin in the coordinate space. The short-range contact interactions and subleading pion-charmed meson couplings are estimated with the phenomenological resonance saturation model. The subleading pion-charmed meson couplings are much weaker than those in the pion-nucleon system, thus the $DD^\ast$ binding mechanism is very different with that of the $NN$ system. We also obtain the analytic structure of the two-pion exchange interactions in the coordinate space, and we find that its asymptotic behavior at long distance is similar to but slightly different with the $NN$ interactions. We get the same asymptotic behavior of the two-pion exchange interaction with that from HAL QCD method but appearing in the longer distance rather than $1 <r<2\text{ fm}$. The binding solution only exists in the isoscalar channel. Our calculation supports the molecular interpretation of $T_{cc}^+$.

==> reply_a.tex <==
Dear Editor,\\

Thank you for handling our manuscript ``$DD^\ast$ chiral interactions with the local momentum-space regularization up to the third order and the molecular nature of $\Tcc$" ({\bf DZ13004/Wang}). We thank the referee
for his/her very valuable comments and suggestions, which will be helpful to improve our manuscript. In the following, we answer the referee's comment item by item.\\

To illustrate the replies and changes clearly, we organize the document as follows:
\begin{itemize}
    \item The referee can click the hyperlink (denoted as, e.g., ``\textcolor{violet}{\bf [C1]}") in the reply to link to the corresponding position of the manuscript.
    \item All the changes in the text are shown in the color \textcolor{red}{RED}. 
\end{itemize}

Sincerely,\\
 
Bo Wang, Lu Meng\\




\noindent\hdashrule[0.5ex]{\textwidth}{0.2mm}{0.9mm 0.45mm}\\
\centerline{Reply to the Referee's Comments and the Summary of Changes Made}\\
\noindent\hdashrule[0.5ex]{\textwidth}{0.2mm}{0.9mm 0.45mm}\\




\setlength{\parindent}{5mm}
%\section{General Comments}

\textbf{(1) Referee's comment:} In the introduction, the author dwelled on some subtle issues one
encountered in computing the TPE NN interactions. However, I would like to
remind the author that some of these issues are alleviated in the covariant
chiral effective field theory, see, e.g., 2111.07766, 2110.05278, 2007.13675.
In these works, it is shown that the TPE contributions are more reasonable even
using the dimensional regularization. These should be mentioned. In addition,
the author may want to show what happens if one does not use the local-momentum
space regularization in the present work.\\

\textbf{Our answer:}
We cited the three papers recommended by the referee in the INTRODUCTION~\cref{covirantEFT}. 

For the last point of this comment: We compared the TPE potentials in local-momentum space regularization and in the unregularzied spectral method, where no regulator is introduced in Sec.~\ref{sec:iiia}. Meanwhile, we compare our potentials with that from recent lattice QCD calculation (HAL QCD collaboration)~[\href{https://arxiv.org/abs/2302.04505}{arXiv: 2302.04505}]. We get the asymptotic behavior $ae^{-2m_\pi r}/r^2$ of the TPE interaction in the long-range limit. However, for the range $1 <r<2$\text{ fm} where HAL QCD obtained the above behavior, our calculations imply that $ae^{-2m_\pi r}/r^n$ with $n>2$ behavior are also very important. Meanwhile, in the local-momentum space regularization, the TPE interaction in the range $1 <r<2$\text{ fm} will depend on the cutoff $\Lambda$~\cref{tpenums}.
\\

\textbf{(2) Referee's comment:} Although the focus of the present work is on the TPE contributions, I found
that the discussions are not adequate. For instance, what are the relative
quantitative importance of the TPE contributions, in comparison with the
contact and OPE interactions. I expect to see a more detailed discussion about
this. At the end, the present work seems to suggest that the TPE contributions
are not important. If this is indeed the case, how important is the OPE
contribution. Anyway, an order-by-order analysis is necessary.\\

\textbf{Our answer:}
We thank the referee for this suggestion. We accordingly added two new subsections, i.e., the Secs.~\ref{sec:iiia} and~\ref{sec:ana}, to derive the asymptotic behavior of the TPE potentials at long distance, and quantitatively analyze the contact, OPE and TPE contributions at each order, as well as the behaviors of the potentials at the short-, long- and intermediate-ranges~\cref{tpenums}.
\\

\textbf{(3) Referee's comment:} The author found that the decay width is larger than the experimental
determination but did not explain why. In Ref.[41] of the present work and many
other similar studies, it was argued that the width of $\Tcc$ as a $DD^\ast$ bound state
is not supposed to be larger than a certain value. I would like to see more
discussions on this issue.\\

\textbf{Our answer:} In the revised version, we considered the complete three-body effect, and in this case, the width of $DD^\ast$ bound state is consistent with the $\Tcc$ (see the discussions in \cref{decaywidth}).\\

\vspace{0.5cm}

{\it We try our best to improve the presentation of the whole manuscript. Finally, we would like to thank the referee again. We hope that the above clarification can answer the referee’s concerns and the present manuscript can meet the standard for publication of PRD.}\\

==> reply_b.tex <==
Dear Editor,\\

Thank you for handling our manuscript ``Revisiting the $DD^\ast$ chiral interactions with the local momentum-space regularization up to the third order and the nature of $\Tcc$" ({\bf DZ13004/Wang}). We thank the referee (B)
for his/her very valuable comments and suggestions, which will be helpful to improve our manuscript. In the following, we answer the referee's comment item by item.

To illustrate the replies and changes clearly, we organize the document as follows:
\begin{itemize}
    \item The referee can click the hyperlink (denoted as, e.g., ``\textcolor{violet}{\bf [C1]}") in the reply to link to the corresponding position of the manuscript.
    \item All the changes in the text are shown in the color \textcolor{red}{RED}. 
\end{itemize}

Sincerely,\\
 
Bo Wang, Lu Meng\\




\noindent\hdashrule[0.5ex]{\textwidth}{0.2mm}{0.9mm 0.45mm}\\
\centerline{Reply to the Referee's Comments and the Summary of Changes Made}\\
\noindent\hdashrule[0.5ex]{\textwidth}{0.2mm}{0.9mm 0.45mm}\\




\setlength{\parindent}{5mm}
%\section{General Comments}

\textbf{(1) Referee's comment:} In the introduction, they review some different approaches on the analysis of the properties of the $T_{cc}$ state.
Among the references, the paper: R. Albuqueque et al., Nucl.Phys.A 1023 (2022) 122451 which improves some predictions quoted by the authors on the $T_{cc}(1^+)$ spectra is missing.\\

\textbf{Our answer:}
We cited the paper recommended by the referee in the INTRODUCTION~\cref{spectra}. 
\\

\textbf{(2) Referee's comment:} The authors quote numbers with decimal in the Tables which do not have too much meaning if the errors for their determinations are not given.\\

\textbf{Our answer:}
We included the errors of the LECs in Tables~\ref{tab:numsci} and \ref{tab:numscii} with the error propagation formula. The error sources come from the parameters in one-boson exchange Lagrangians that quoted in the appendix. The numerical results are more sensitive to the cutoff, so we present the results with the central values of LECs via varying the cutoff in a reasonable range.
\\

\textbf{(3) Referee's comment:} Some other relevant papers on the determination of $M_{\sigma}$ from $\pi\pi$ and $\gamma\gamma$ scattering are missing (F.J Yndurain et al, Phys.Rev.D 76 (2007) 074034; G. Mennesier et al. Phys.Lett.B 665 (2008) 205).\\

\textbf{Our answer:} We cited the papers recommended by the referee in the Appendix~\ref{sec:app}~\cref{refsig}.\\

\textbf{(4) Referee's comment:} Most of the results (e.g shape of the potential) depend strongly on the value of the cut-off $\Lambda$ at which $\chi$EFT breakdown though one would expect that physical observables should be independent of it. Can the authors clarify this point ?\\

\textbf{Our answer:} As pointed by the referee, the physical observables should in principle be independent on the regularization scale $\Lambda$. However, how to get rid of the cutoff dependence reasonably in nonperturbative calculations is still an debatable problem even for the nucleon systems~\cite{Gasparyan:2022isg}. In practices, two ways are usually used: (1) Fitting the unknown LECs via varying the cutoff in a range if the corresponding experimental data are adequate (such as the $NN$ scatterings). In this case, the cutoff dependence is largely absorbed by the LECs, which makes the physical observables from high order calculation become very insensitive to the cutoff. (2) If the experimental data are not adequate (e.g., the $DD^\ast$ case in this work), one may resort to some phenomenological approaches to estimate the LECs (such as the resonance saturation model). In this case, the physical quantities would be cutoff dependent, but one can still get some meaningful conclusions as long as the cutoff is chosen in a reasonable range regarding the sepcific EFT. In $\chi$EFT, the cutoff is around $500$ MeV~\cite{Epelbaum:2008ga,Machleidt:2011zz}, so in our study we analyzed the behaviors of effective potentials via taking $\Lambda\in[400,700]$ MeV, and we also found that the binding solution of $DD^\ast$ system appears when $\Lambda\simeq520$ MeV.\\

%\vspace{0.2cm}

{\it We try our best to improve the presentation of the whole manuscript. Finally, we would like to thank the referee again. We hope that the above clarification can answer the referee’s concerns and the present manuscript can meet the standard for publication of PRD.}\\
